Erlangen Program at Large--2: Inventing a wheel. The parabolic one

We discuss parabolic versions of Euler's identity e^{it}=cos t + i sin t. A purely algebraic approach based on dual numbers is known to produce a very trivial relation e^{pt} = 1+pt. Therefore we use a geometric setup of parabolic rotations to recover the corresponding non-trivial algebraic framework. Our main tool is Moebius transformations which turn out to be closely related to induced representations of the group SL(2,R). Keywords: complex numbers, dual numbers, double numbers, linear algebra, invariant, computer algebra, GiNaC

==> mydef.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%       $Id: mydef.tex,v 1.35 2007/03/07 10:43:52 kisilv Exp kisilv $    
%
%  File mydef.tex
%
\typeout{This is MyDef macros file}
\makeatletter
\def\ifundefined#1{\expandafter\ifx\csname#1\endcsname\relax}
\hyphenation{di-men-sio-nal}
%% Do not uncomment---does not work
%\ifundefined{tthtrue}
%  \newif\iftth
%\fi
\providecommand{\comment}[1]{}
\def\smnegskip{\mskip-0.6\thinmuskip}
\usepackage{amsfonts}
\providecommand{\tthdump}[1]{#1}
\tthdump{\newlength{\curmathsize}}
%
%   Objects
%
\providecommand{\algebra}[1]{\ensuremath{\mathfrak{#1}}}
\providecommand{\Heisen}[1]{{\ensuremath{\mathbb{H}^{#1}}}}
\providecommand{\hHeisen}[1]{\ensuremath{\widehat{\mathbb {H}}^{#1}}}
\providecommand{\Cliff}[2][\comment]{{\ensuremath{%
\mathcal{C}\kern-0.18em\ell(#1,#2)}}}
%\providecommand{\Cliff}[2][\comment]{\ensuremath{\mathbf{Cl}(#1,#2)}}
\providecommand{\object}[2][\,]{\ensuremath{\mathrm{#2}#1}}
\providecommand{\Space}[3][]{\ensuremath{\mathbb{#2}^{#3}_{#1}{}}}
\providecommand{\such}{\,\mid\,}
\providecommand{\Jacobian}[1]{\ensuremath{\mathcal{J}(#1)}}
\iftth
  \providecommand{\FSpace}[3][]{\ensuremath{#2_{#3}^{#1}{}}} 
  \providecommand{\limlike}[1]{\mathop{#1}}
  \providecommand{\loglike}[1]{\mathrm{#1}}
\else
  \providecommand{\FSpace}[3][]{\ensuremath{\ifx#2l \ell_{#3}^{#1}{}\else
  #2_{#3}^{#1}{}\fi}} 
  \providecommand{\limlike}[1]{\mathop {\operator@font #1}}
  \providecommand{\loglike}[1]{\mathop {\operator@font #1}\nolimits}
\fi
\providecommand{\Quater}{\ensuremath{\mathcal{H}}}
\providecommand{\bos}{\mathcal{B}}
\ifundefined{qed}
    \DeclareMathSymbol{\qed}{0}{AMSa}{"03}
\fi
\providecommand{\SL}[1][2]{\ensuremath{\FSpace{SL}{#1}(\Space{R}{})}}
%
%  Unary operations
%
\providecommand{\fourier}[1]{\ensuremath{\mathcal{F}^{#1}{}}}
\providecommand{\bra}[1]{\ensuremath{\left\langle#1\right|}}
\providecommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
\providecommand{\Cplus}{\ensuremath{C^{+}}}
\providecommand{\Cstar}{\ensuremath{C^{*}}}
\providecommand{\onvol}{^{+}}
\providecommand{\spec}[1][]{\ensuremath{\mathbf{sp}}\,}
\providecommand{\sr}{\ensuremath{\mathbf{r}}\,}
\providecommand{\kernel}{\ensuremath{\mathbf{ker}}\,}
\providecommand{\ad}{\ensuremath{\mathbf{ad}}\,}
\providecommand{\diag}{\mathop {\operator@font diag}\nolimits}
\providecommand{\norm}[2][\relax]{\left\|#2\right\|\ifx#1\relax\else_{#1}\fi}
\providecommand{\modulus}[2][\relax]{\left| #2 \right|\ifx#1\relax\else_{#1}\fi}
\providecommand{\oper}[1]{\mathcal{#1}}
\providecommand{\rmi}{\mathrm{i}}
\providecommand{\rme}{\mathrm{e}}
\providecommand{\rmh}{\epsilon}
\providecommand{\rmp}{\varepsilon}
\providecommand{\tr}{\mathop{tr}}

%
%  Binary operations%
\providecommand{\scalar}[3][\relax]{\left\langle #2,#3 
        \right\rangle\ifx#1\relax\else_{#1}\fi}
\providecommand{\intersect}[2]{\left.#1\right|_{#2}}
\providecommand{\relstack}[2]{{\mathrel {\mathop {#1}\limits _{#2}}}}
%
%
%
\providecommand{\eqref}[1]{\textup{(\ref{#1})}}
\providecommand{\eqnright}[1]{\qquad\qquad  #1}
\providecommand{\person}[1]{\textsc{#1}}
%
%  WWW commands
%
\providecommand{\href}[2]{#2}
\iftth
  \special{html:<BODY BGCOLOR=ffffff>}
  \providecommand{\MR}[1]{%
\textbf{MR}~\special{html:<a
href="http://www.ams.org/mathscinet-getitem?mr=#1">\# #1</a>}}
  \providecommand{\Zbl}[1]{%
\textbf{Zbl}~\special{html:<a
href="http://www.emis.de:80/cgi-bin/zmen/ZMATH/en/zmathf.html?first=1&maxdocs=3&type=html&an=#1&format=complete">\#
#1</a>}}
\else
    \ifundefined{MR}
        \providecommand{\MR}[1]{\textbf{MR}~\href{http://www.ams.org/mathscinet-getitem?mr=#1}{\#~#1}}
    \else
        \renewcommand{\MR}[1]{\textbf{MR}~\href{http://www.ams.org/mathscinet-getitem?mr=#1}{\#~#1}}
    \fi
  \providecommand{\Zbl}[1]{\textbf{Zbl}~\href{http://www.emis.de:80/cgi-bin/zmen/ZMATH/en/zmathf.html?first=1&maxdocs=3&type=html&an=#1&format=complete}{\#~#1}}
\fi

\providecommand{\myeprint}[2]{E-print: \href{#1}{\texttt{#2}}}
\providecommand{\mailto}[1]{\href{mailto:#1}{\texttt{#1}}}
\providecommand{\urltt}[1]{\href{#1}{\texttt{#1}}}

\newif\ifrawhtml
\newenvironment{rawhtml}{\ifrawhtml}{\fi}
%
\makeatother
\endinput

